Unifying Linearity and Dependency Analyses

Linearity and dependency analyses are key to several applications in computer science, especially, in resource management and information flow control. What connects these analyses is that both of them need to model at least two different worlds with constrained mutual interaction. Though linearity and dependency analyses address similar problems, the analyses are carried out by employing different methods. For linearity analysis, type systems employ the comonadic exponential modality from Girard's linear logic. For dependency analysis, type systems employ the monadic modality from Moggi's computational metalanguage. Owing to this methodical difference, a unification of the two analyses, though theoretically and practically desirable, is not straightforward. Fortunately, with recent advances in graded-context type systems, it has been realized that linearity and dependency analyses can be viewed through the same lens. However, existing graded-context type systems fall short of a unification of linearity and dependency analyses. The problem with existing graded-context type systems is that though their linearity analysis is general, their dependency analysis is limited, primarily because the graded modality they employ is comonadic and not monadic. In this paper, we address this limitation by systematically extending existing graded-context type systems so that the graded modality is both comonadic and monadic. This extension enables us to unify linearity analysis with a general dependency analysis. We present a unified Linear Dependency Calculus, LDC, which analyses linearity and dependency using the same mechanism in an arbitrary Pure Type System. We show that LDC is a general linear and dependency calculus by subsuming into it the standard calculi for the individual analyses.

==> Makefile <==
all : paper.pdf

RULESFILE = Rules.tex

OTT_SOURCE = Rules.ott
OTTIFLAGS = $(foreach i, $(OTT_SOURCE), -i $(i))
PAPER_MNG = $(wildcard Sections/*.mng)
PAPER_SOURCE = $(patsubst %.mng,%.tex,$(PAPER_MNG))
OTT_FILTER := $(subst .mng,.mng ,$(addprefix -tex_filter ,$(join $(PAPER_MNG), $(PAPER_SOURCE))))

Sections/%.tex : $(RULESFILE) Sections/%.mng Makefile
	rm -f $(PAPER_SOURCE)
	ott -tex_wrap false \
            -tex_show_meta false \
	    $(OTTIFLAGS) \
            $(OTT_FILTER)
	chmod a-w $(PAPER_SOURCE)

$(RULESFILE) : $(OTT_SOURCE)
	ott -tex_wrap false -i $(OTT_SOURCE) -o $(RULESFILE)

paper.pdf : paper.tex Rules.tex Biblio.bib Sections/Abstract.tex $(PAPER_SOURCE)
	latexmk -pdf -bibtex paper.tex; rm *.aux *.out *.fls *.fdb_latexmk

clean :
	rm -f *.aux *.out *.fls *.fdb_latexmk *.pdf *.bbl



==> Sections/Related.tex <==
\section{Discussions}

\subsection{Dependent Types and Linearity Analysis}

Linear and dependent types have an interesting history of relationship. Initially, they were thought to be incompatible. Their incompatibility was succinctly captured in the principle: `types can not depend upon linear variables', enforced by all the linear dependent type systems \cite[etc]{cervesato,krishna,vakar} proposed earlier. Later, \cite{mcbride} challenged this principle and showed that linear and dependent types can be seamlessly combined with one another. In McBride's system, types can indeed depend upon linear variables. McBride's work inspired several linear dependent type systems \cite{atkey,grad,moon} that vary in how they track usage in types. Among these systems, \Bw{} is close to the system \textsc{GraD}, proposed by \cite{grad}.

\textsc{GraD} is a general coeffect calculus parametrized by an arbitrary partially-ordered semiring. \Bw{}, on the other hand, tracks linearity and is parametrized by the partially-ordered semiring $\mathbb{N}^{\omega} = (\mathbb{N} \cup \{  \omega  \}, + , 0 , \cdot , 1 ,  <:  )$. When compared over this semiring $\mathbb{N}^{\omega}$, \Bw{} subsumes \textsc{GraD}. We express this subsumption as a theorem below.

\begin{theorem}\label{GraD}
With $\mathbb{N}^{\omega}$ as the parametrizing partially-ordered semiring, if $ \Gamma  \vdash  \ottnt{a}  : \:  \ottnt{A} $ in \textsc{GraD}, then $ \Gamma  \vdash  \ottnt{a}  :^{  1  }  \ottnt{A} $ in \Bw{}. Further, if $ \vdash  \ottnt{a}  \leadsto  \ottnt{a'} $ in \textsc{GraD}, then $ \vdash  \ottnt{a}  \leadsto  \ottnt{a'} $ in \Bw{}.
\end{theorem} 

Hence, with regard to linearity analysis, \Bw{} is at least as expressive as \textsc{GraD}.        

\subsection{Dependent Types and Dependency Analysis}

Dependency analysis and dependent types have come together only sparingly \cite{prost,color,ddc}. Among the type systems that combine the two, $\text{DDC}^{\top}$, proposed by \cite{ddc}, is the closest to \Bw{}. In fact, \Bw{}, seen as a dependency calculus, subsumes $\text{DDC}^{\top}$. We express this subsumption as a theorem below.
 
\begin{theorem} \label{DDCT}
With $\mathcal{L}$ as the parametrizing lattice, if $ \Gamma  \vdash  \ottnt{a}  :^{ \ell }  \ottnt{A} $ in $\text{DDC}^{\top}$, then $ \Gamma  \vdash  \ottnt{a}  :^{ \ell }  \ottnt{A} $ in \Bw{}. Further, if $ \vdash  \ottnt{a}  \leadsto  \ottnt{a'} $ in $\text{DDC}^{\top}$, then $ \vdash  \ottnt{a}  \leadsto  \ottnt{a'} $ in \Bw{}.
\end{theorem}

Hence, with regard to dependency analysis, \Bw{} is at least as expressive as $\text{DDC}^{\top}$.
\iffalse
\subsection{Linearity Analysis and Dependency Analysis}

We showed that bounded linearity analysis and dependency analysis are essentially the same analysis viewed from two different angles. This observation has a precedent: \cite{linearmonad} showed that models of linear logic also provide models of Moggi's computational $\lambda$-calculus. Broadly speaking, bounded linear logic is fine-grained linear logic and dependency calculus is fine-grained computational $\lambda$-calculus. So our result may be seen as a generalization of that of \cite{linearmonad}.

Linearity has usually been analyzed as a coeffect whereas dependency as an effect. Analysis of effects and coeffects have come together in some existing work \cite{effcoeff,rajani}. However, existing work generally uses different modalities for representing effects and coeffects and then combines them either via distributive laws as in \cite{effcoeff} or via potentials as in \cite{rajani}. We, on the other hand, use the same modality for representing effects and coeffects. While such a treatment of effects and coeffects may not be possible in general, we show that it is possible for interactions like resource usage and information flow.     
\fi

% tracks both resource usage and information flow using the same mechanismWhen we take their dual nature into account in our analyses, we understand more of their nuances. We also understand more how they relate to one another. With this understanding, we can unify some analyses into a single analysis. In this paper, we unified resource usage and information flow analyses into a single calculus, BLDC. Using a heap semantics, we modeled interaction of programs, derived in this calculus, with their environments. From soundness of the calculus with respect to this heap semantics, we concluded that it analyzes resource usage and information flow correctly. This calculus gives us a new perspective on resource usage, as we see in the simplified presentation of linear nonlinear logic. This calculus also relates some of the existing calculi tracking either resource usage or information flow. 

%Linear and dependent types have come together in several type systems . Such type systems usually have an LNL style of analyzing linearity. The LNL style that works smoothly in a simply-typed setting poses a problem in the dependent setting \cite{mcbride}. In this style, linear assumptions from two different premise judgments are concatenated in the conclusion judgment in some of the typing rules. Such a concatenation is problematic in a dependent setting because types appearing later in a context may depend upon earlier assumptions. \cite{mcbride} solved this problem by introducing $0$ use to the existing linear and nonlinear uses permitted by LNL style calculi. McBride's calculus is quite general in that it is parametrized by an arbitrary semiring. BLDC is similar to McBride's calculus. However, BLDC is not parametrized by an arbitrary semiring. In fact, such a parametrization leads to failure of substitution \cite{atkey}. Several type systems  were proposed in response to the failure of substitution in McBride's calculus. But all these systems kept the parametrizing structure intact and put restrictions on the form of the typing judgment. We went the other way and put restrictions on the parametrizing structure while keeping the form of the typing judgment intact.

   
